Offline Policy Comparison with Confidence: Benchmarks and Baselines

Decision makers often wish to use offline historical data to compare sequential-action policies at various world states. Importantly, computational tools should produce confidence values for such offline policy comparison (OPC) to account for statistical variance and limited data coverage. Nevertheless, there is little work that directly evaluates the quality of confidence values for OPC. In this work, we address this issue by creating benchmarks for OPC with Confidence (OPCC), derived by adding sets of policy comparison queries to datasets from offline reinforcement learning. In addition, we present an empirical evaluation of the risk versus coverage trade-off for a class of model-based baselines. In particular, the baselines learn ensembles of dynamics models, which are used in various ways to produce simulations for answering queries with confidence values. While our results suggest advantages for certain baseline variations, there appears to be significant room for improvement in future work.

==> assets/query-eval/gym-mujoco/mixture/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{mixture} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-mixture}
\begin{center} 
\begin{footnotesize} 
\begin{sc}
    \begin{tabular}{|l | c | c | c| c | c | c |}
        \toprule
        Env. & mixture & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ \\
        \midrule
        Half\\Cheetah & False & $0.219\pm0.005$ & $0.044\pm0.005$ & $0.46\pm0.04$ & $0.374\pm0.004$ \\
        \midrule
        Hopper & False & $0.141\pm0.005$ & $0.031\pm0.005$ & $0.428\pm0.034$ & $0.268\pm0.004$ \\
        \midrule
        Walker\\2d & False & $0.068\pm0.001$ & $0.011\pm0.003$ & $0.3\pm0.051$ & $0.159\pm0.002$ \\
        \bottomrule
    \end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/gym-mujoco/mixture/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.7]{assets/query-eval/gym-mujoco/mixture/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{mixture} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-mixture}
\end{figure}

==> assets/query-eval/maze/mixture/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{mixture} comparison in \emph{maze} environments } 
\label{table:maze-mixture}
\begin{center} 
\begin{footnotesize} 
\begin{sc}
    \begin{tabular}{|l | c | c | c| c | c | c |}
        \toprule
        Env. & mixture & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ \\
        \midrule
        large & False & $0.14\pm0.015$ & $0.062\pm0.004$ & $0.82\pm0.035$ & $0.251\pm0.029$ \\
        \midrule
        medium & False & $0.001\pm(<0.001)$ & $0.0\pm(<0.001)$ & $0.2\pm(<0.001)$ & $0.022\pm0.001$ \\
        \midrule
        open & False & $0.029\pm0.001$ & $0.012\pm0.001$ & $0.5\pm(<0.001)$ & $0.107\pm0.005$ \\
        \midrule
        umaze & False & $0.008\pm0.001$ & $0.002\pm(<0.001)$ & $0.3\pm(<0.001)$ & $0.075\pm0.003$ \\
        \bottomrule
    \end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/maze/mixture/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.7]{assets/query-eval/maze/mixture/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{mixture} in \emph{maze} environments } 
\label{fig:maze-mixture}
\end{figure}

==> assets/query-eval/old-tables-with-std/gym-mujoco/dataset-quality/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{dataset-quality} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-dataset-quality}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & dataset-quality & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{5}{3.6em}{Half\\Cheetah}  & expert & $0.212\pm0.0$ & $0.05\pm0.0$ & $0.5\pm0.0$ & $0.361\pm0.0$ & 5 \\ 
& medium & $0.222\pm0.0$ & $0.048\pm0.0$ & $0.5\pm0.0$ & $0.374\pm0.0$ & 5 \\ 
& medium-expert & $0.24\pm0.0$ & $0.06\pm0.0$ & $0.6\pm0.0$ & $0.387\pm0.0$ & 5 \\ 
& medium-replay & $0.216\pm0.0$ & $0.04\pm0.0$ & $0.4\pm0.0$ & $0.368\pm0.0$ & 5 \\ 
& random & $0.206\pm0.0$ & $0.023\pm0.0$ & $0.3\pm0.0$ & $0.378\pm0.0$ & 5 \\ 
\midrule 
\multirow{5}{3.6em}{Hopper}  & expert & $0.152\pm0.0$ & $0.04\pm0.0$ & $0.5\pm0.0$ & $0.284\pm0.0$ & 5 \\ 
& medium & $0.133\pm0.0$ & $0.03\pm0.0$ & $0.4\pm0.0$ & $0.26\pm0.0$ & 5 \\ 
& medium-expert & $0.136\pm0.0$ & $0.028\pm0.0$ & $0.4\pm0.0$ & $0.265\pm0.0$ & 5 \\ 
& medium-replay & $0.128\pm0.0$ & $0.012\pm0.0$ & $0.3\pm0.0$ & $0.258\pm0.0$ & 5 \\ 
& random & $0.156\pm0.01$ & $0.045\pm0.0$ & $0.54\pm0.05$ & $0.273\pm0.0$ & 5 \\ 
\midrule 
\multirow{5}{3.6em}{Walker\\2d}  & expert & $0.064\pm0.0$ & $0.011\pm0.0$ & $0.3\pm0.0$ & $0.161\pm0.0$ & 5 \\ 
& medium & $0.069\pm0.0$ & $0.007\pm0.0$ & $0.22\pm0.04$ & $0.156\pm0.0$ & 5 \\ 
& medium-expert & $0.068\pm0.0$ & $0.007\pm0.0$ & $0.24\pm0.05$ & $0.153\pm0.0$ & 5 \\ 
& medium-replay & $0.07\pm0.0$ & $0.005\pm0.0$ & $0.2\pm0.0$ & $0.161\pm0.0$ & 5 \\ 
& random & $0.067\pm0.0$ & $0.024\pm0.0$ & $0.54\pm0.05$ & $0.165\pm0.0$ & 5 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/gym-mujoco/dataset-quality/sr_coverage.tex <==
\begin{figure}[!h]
\centering
\includegraphics[scale=0.66]{assets/query-eval/gym-mujoco/dataset-quality/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{dataset-quality} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-dataset-quality}
\end{figure}

==> assets/query-eval/old-tables-with-std/gym-mujoco/deterministic/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{deterministic} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-deterministic}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & deterministic & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{2}{3.6em}{Half\\Cheetah}  & False & $0.229\pm0.02$ & $0.054\pm0.01$ & $0.568\pm0.15$ & $0.377\pm0.01$ & 25 \\ 
& True & $0.219\pm0.01$ & $0.044\pm0.01$ & $0.46\pm0.1$ & $0.374\pm0.01$ & 25 \\ 
\midrule 
\multirow{2}{3.6em}{Hopper}  & False & $0.138\pm0.0$ & $0.039\pm0.01$ & $0.524\pm0.1$ & $0.26\pm0.01$ & 25 \\ 
& True & $0.141\pm0.01$ & $0.031\pm0.01$ & $0.428\pm0.09$ & $0.268\pm0.01$ & 25 \\ 
\midrule 
\multirow{2}{3.6em}{Walker\\2d}  & False & $0.064\pm0.0$ & $0.012\pm0.0$ & $0.328\pm0.06$ & $0.16\pm0.01$ & 25 \\ 
& True & $0.068\pm0.0$ & $0.011\pm0.01$ & $0.3\pm0.13$ & $0.159\pm0.0$ & 25 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/gym-mujoco/deterministic/sr_coverage.tex <==
\begin{figure}[!h]
\centering
\includegraphics[scale=0.66]{assets/query-eval/gym-mujoco/deterministic/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{deterministic} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-deterministic}
\end{figure}

==> assets/query-eval/old-tables-with-std/gym-mujoco/dynamics-type/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{dynamics-type} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-dynamics-type}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & dynamics-type & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{2}{3.6em}{Half\\Cheetah}  & autoregressive & $0.249\pm0.02$ & $0.068\pm0.02$ & $0.736\pm0.22$ & $0.379\pm0.01$ & 25 \\ 
& feed-forward & $0.219\pm0.01$ & $0.044\pm0.01$ & $0.46\pm0.1$ & $0.374\pm0.01$ & 25 \\ 
\midrule 
\multirow{2}{3.6em}{Hopper}  & autoregressive & $0.139\pm0.02$ & $0.034\pm0.01$ & $0.48\pm0.11$ & $0.268\pm0.02$ & 25 \\ 
& feed-forward & $0.141\pm0.01$ & $0.031\pm0.01$ & $0.428\pm0.09$ & $0.268\pm0.01$ & 25 \\ 
\midrule 
\multirow{2}{3.6em}{Walker\\2d}  & autoregressive & $0.065\pm0.0$ & $0.013\pm0.01$ & $0.356\pm0.12$ & $0.158\pm0.0$ & 25 \\ 
& feed-forward & $0.068\pm0.0$ & $0.011\pm0.01$ & $0.3\pm0.13$ & $0.159\pm0.0$ & 25 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/gym-mujoco/dynamics-type/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.66]{assets/query-eval/gym-mujoco/dynamics-type/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{dynamics-type} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-dynamics-type}
\end{figure}

==> assets/query-eval/old-tables-with-std/gym-mujoco/ensemble-count/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{ensemble-count} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-ensemble-count}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & ensemble-count & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{5}{3.6em}{Half\\Cheetah}  & 10 & $0.209\pm0.01$ & $0.028\pm0.01$ & $0.32\pm0.07$ & $0.378\pm0.01$ & 25 \\ 
& 20 & $0.213\pm0.01$ & $0.034\pm0.01$ & $0.36\pm0.1$ & $0.376\pm0.01$ & 25 \\ 
& 40 & $0.215\pm0.01$ & $0.039\pm0.01$ & $0.4\pm0.09$ & $0.374\pm0.01$ & 25 \\ 
& 80 & $0.219\pm0.01$ & $0.043\pm0.01$ & $0.452\pm0.1$ & $0.374\pm0.01$ & 25 \\ 
& 100 & $0.219\pm0.01$ & $0.044\pm0.01$ & $0.46\pm0.1$ & $0.374\pm0.01$ & 25 \\ 
\midrule 
\multirow{5}{3.6em}{Hopper}  & 10 & $0.141\pm0.01$ & $0.02\pm0.01$ & $0.316\pm0.07$ & $0.273\pm0.01$ & 25 \\ 
& 20 & $0.141\pm0.01$ & $0.024\pm0.01$ & $0.344\pm0.09$ & $0.272\pm0.01$ & 25 \\ 
& 40 & $0.141\pm0.01$ & $0.027\pm0.01$ & $0.388\pm0.1$ & $0.27\pm0.01$ & 25 \\ 
& 80 & $0.141\pm0.01$ & $0.03\pm0.01$ & $0.416\pm0.1$ & $0.269\pm0.01$ & 25 \\ 
& 100 & $0.141\pm0.01$ & $0.031\pm0.01$ & $0.428\pm0.09$ & $0.268\pm0.01$ & 25 \\ 
\midrule 
\multirow{5}{3.6em}{Walker\\2d}  & 10 & $0.072\pm0.0$ & $0.007\pm0.0$ & $0.256\pm0.08$ & $0.16\pm0.01$ & 25 \\ 
& 20 & $0.071\pm0.0$ & $0.008\pm0.01$ & $0.268\pm0.1$ & $0.16\pm0.01$ & 25 \\ 
& 40 & $0.07\pm0.0$ & $0.01\pm0.01$ & $0.28\pm0.12$ & $0.16\pm0.0$ & 25 \\ 
& 80 & $0.068\pm0.0$ & $0.01\pm0.01$ & $0.284\pm0.13$ & $0.159\pm0.0$ & 25 \\ 
& 100 & $0.068\pm0.0$ & $0.011\pm0.01$ & $0.3\pm0.13$ & $0.159\pm0.0$ & 25 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/gym-mujoco/ensemble-count/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.6]{assets/query-eval/gym-mujoco/ensemble-count/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{ensemble-count} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-ensemble-count}
\end{figure}

==> assets/query-eval/old-tables-with-std/gym-mujoco/horizon/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{horizon} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-horizon}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & horizon & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{5}{3.6em}{Half\\Cheetah}  & 10.0 & $0.077\pm0.01$ & $0.008\pm0.0$ & $0.288\pm0.04$ & $0.191\pm0.02$ & 25 \\ 
& 20.0 & $0.217\pm0.02$ & $0.041\pm0.01$ & $0.416\pm0.11$ & $0.374\pm0.01$ & 25 \\ 
& 30.0 & $0.215\pm0.01$ & $0.038\pm0.01$ & $0.404\pm0.1$ & $0.377\pm0.01$ & 25 \\ 
& 40.0 & $0.223\pm0.01$ & $0.049\pm0.02$ & $0.464\pm0.11$ & $0.368\pm0.01$ & 25 \\ 
& 50.0 & $0.277\pm0.02$ & $0.063\pm0.02$ & $0.516\pm0.14$ & $0.428\pm0.01$ & 25 \\ 
\midrule 
\multirow{5}{3.6em}{Hopper}  & 10.0 & $0.017\pm0.01$ & $0.001\pm0.0$ & $0.2\pm0.0$ & $0.048\pm0.01$ & 25 \\ 
& 20.0 & $0.078\pm0.0$ & $0.016\pm0.01$ & $0.336\pm0.1$ & $0.17\pm0.01$ & 25 \\ 
& 30.0 & $0.146\pm0.01$ & $0.029\pm0.01$ & $0.42\pm0.08$ & $0.284\pm0.01$ & 25 \\ 
& 40.0 & $0.169\pm0.02$ & $0.038\pm0.01$ & $0.432\pm0.09$ & $0.293\pm0.01$ & 25 \\ 
& 50.0 & $0.196\pm0.02$ & $0.047\pm0.02$ & $0.516\pm0.13$ & $0.334\pm0.01$ & 25 \\ 
\midrule 
\multirow{5}{3.6em}{Walker\\2d}  & 10.0 & $0.011\pm0.0$ & $0.001\pm0.0$ & $0.22\pm0.04$ & $0.033\pm0.01$ & 25 \\ 
& 20.0 & $0.025\pm0.0$ & $0.003\pm0.0$ & $0.252\pm0.11$ & $0.077\pm0.01$ & 25 \\ 
& 30.0 & $0.059\pm0.0$ & $0.01\pm0.01$ & $0.3\pm0.15$ & $0.132\pm0.01$ & 25 \\ 
& 40.0 & $0.093\pm0.0$ & $0.017\pm0.01$ & $0.384\pm0.13$ & $0.209\pm0.01$ & 25 \\ 
& 50.0 & $0.131\pm0.0$ & $0.023\pm0.01$ & $0.392\pm0.15$ & $0.259\pm0.0$ & 25 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/gym-mujoco/horizon/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.63]{assets/query-eval/gym-mujoco/horizon/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{horizon} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-horizon}
\end{figure}

==> assets/query-eval/old-tables-with-std/gym-mujoco/mixture/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{mixture} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-mixture}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & mixture & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
Half\\Cheetah & False & $0.219\pm0.01$ & $0.044\pm0.01$ & $0.46\pm0.1$ & $0.374\pm0.01$ & 25 \\ 
\midrule 
Hopper & False & $0.141\pm0.01$ & $0.031\pm0.01$ & $0.428\pm0.09$ & $0.268\pm0.01$ & 25 \\ 
\midrule 
Walker\\2d & False & $0.068\pm0.0$ & $0.011\pm0.01$ & $0.3\pm0.13$ & $0.159\pm0.0$ & 25 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/gym-mujoco/mixture/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.7]{assets/query-eval/gym-mujoco/mixture/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{mixture} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-mixture}
\end{figure}

==> assets/query-eval/old-tables-with-std/gym-mujoco/normalization/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{normalize} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-normalize}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & normalize & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{2}{3.6em}{Half\\Cheetah}  & False & $0.228\pm0.02$ & $0.053\pm0.02$ & $0.548\pm0.18$ & $0.376\pm0.01$ & 25 \\ 
& True & $0.219\pm0.01$ & $0.044\pm0.01$ & $0.46\pm0.1$ & $0.374\pm0.01$ & 25 \\ 
\midrule 
\multirow{2}{3.6em}{Hopper}  & False & $0.128\pm0.01$ & $0.017\pm0.01$ & $0.3\pm0.06$ & $0.255\pm0.01$ & 25 \\ 
& True & $0.141\pm0.01$ & $0.031\pm0.01$ & $0.428\pm0.09$ & $0.268\pm0.01$ & 25 \\ 
\midrule 
\multirow{2}{3.6em}{Walker\\2d}  & False & $0.078\pm0.02$ & $0.013\pm0.01$ & $0.316\pm0.19$ & $0.17\pm0.02$ & 25 \\ 
& True & $0.068\pm0.0$ & $0.011\pm0.01$ & $0.3\pm0.13$ & $0.159\pm0.0$ & 25 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/gym-mujoco/normalization/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.66]{assets/query-eval/gym-mujoco/normalization/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{normalize} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-normalize}
\end{figure}

==> assets/query-eval/old-tables-with-std/gym-mujoco/prior-scale/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{prior-scale} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-prior-scale}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & prior-scale & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{2}{3.6em}{Half\\Cheetah}  & 0 & $0.219\pm0.01$ & $0.044\pm0.01$ & $0.46\pm0.1$ & $0.374\pm0.01$ & 25 \\ 
& 5 & $0.236\pm0.01$ & $0.067\pm0.01$ & $0.768\pm0.21$ & $0.373\pm0.01$ & 25 \\ 
\midrule 
\multirow{2}{3.6em}{Hopper}  & 0 & $0.141\pm0.01$ & $0.031\pm0.01$ & $0.428\pm0.09$ & $0.268\pm0.01$ & 25 \\ 
& 5 & $0.145\pm0.01$ & $0.045\pm0.01$ & $0.616\pm0.13$ & $0.269\pm0.01$ & 25 \\ 
\midrule 
\multirow{2}{3.6em}{Walker\\2d}  & 0 & $0.068\pm0.0$ & $0.011\pm0.01$ & $0.3\pm0.13$ & $0.159\pm0.0$ & 25 \\ 
& 5 & $0.057\pm0.0$ & $0.017\pm0.0$ & $0.44\pm0.1$ & $0.159\pm0.0$ & 25 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/gym-mujoco/prior-scale/sr_coverage.tex <==
\begin{figure}[!h]
\centering
\includegraphics[scale=0.66]{assets/query-eval/gym-mujoco/prior-scale/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{prior-scale} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-prior-scale}
\end{figure}

==> assets/query-eval/old-tables-with-std/gym-mujoco/uncertainty-type/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{uncertainty-type} comparison in \emph{gym-mujoco} environments } 
\label{table:gym-mujoco-uncertainty-type}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & uncertainty-type & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{3}{3.6em}{Half\\Cheetah}  & ev & $0.219\pm0.01$ & $0.044\pm0.01$ & $0.46\pm0.1$ & $0.374\pm0.01$ & 25 \\ 
& pci & $0.191\pm0.01$ & $0.006\pm0.0$ & $0.2\pm0.0$ & $0.373\pm0.01$ & 25 \\ 
& u-pci & $0.196\pm0.01$ & $0.014\pm0.0$ & $0.228\pm0.04$ & $0.373\pm0.01$ & 25 \\ 
\midrule 
\multirow{3}{3.6em}{Hopper}  & ev & $0.141\pm0.01$ & $0.031\pm0.01$ & $0.428\pm0.09$ & $0.268\pm0.01$ & 25 \\ 
& pci & $0.135\pm0.01$ & $0.004\pm0.0$ & $0.2\pm0.0$ & $0.269\pm0.01$ & 25 \\ 
& u-pci & $0.135\pm0.01$ & $0.009\pm0.0$ & $0.216\pm0.04$ & $0.269\pm0.01$ & 25 \\ 
\midrule 
\multirow{3}{3.6em}{Walker\\2d}  & ev & $0.068\pm0.0$ & $0.011\pm0.01$ & $0.3\pm0.13$ & $0.159\pm0.0$ & 25 \\ 
& pci & $0.078\pm0.0$ & $0.002\pm0.0$ & $0.2\pm0.0$ & $0.16\pm0.01$ & 25 \\ 
& u-pci & $0.076\pm0.0$ & $0.004\pm0.0$ & $0.22\pm0.04$ & $0.16\pm0.01$ & 25 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/gym-mujoco/uncertainty-type/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.66]{assets/query-eval/gym-mujoco/uncertainty-type/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{uncertainty-type} in \emph{gym-mujoco} environments } 
\label{fig:gym-mujoco-uncertainty-type}
\end{figure}

==> assets/query-eval/old-tables-with-std/maze/dataset-quality/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{dataset-quality} comparison in \emph{maze} environments } 
\label{table:maze-dataset-quality}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & dataset-quality & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
large & 1m & $0.14\pm0.02$ & $0.062\pm0.0$ & $0.82\pm0.04$ & $0.251\pm0.03$ & 5 \\ 
\midrule 
medium & 1m & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.022\pm0.0$ & 5 \\ 
\midrule 
open & 1m & $0.029\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.107\pm0.01$ & 5 \\ 
\midrule 
umaze & 1m & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.075\pm0.0$ & 5 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/maze/dataset-quality/sr_coverage.tex <==
\begin{figure}[!h]
\centering
\includegraphics[scale=0.66]{assets/query-eval/maze/dataset-quality/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{dataset-quality} in \emph{maze} environments } 
\label{fig:maze-dataset-quality}
\end{figure}

==> assets/query-eval/old-tables-with-std/maze/deterministic/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{deterministic} comparison in \emph{maze} environments } 
\label{table:maze-deterministic}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & deterministic & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{2}{3.6em}{large}  & False & $0.152\pm0.01$ & $0.058\pm0.01$ & $0.54\pm0.05$ & $0.167\pm0.0$ & 5 \\ 
& True & $0.14\pm0.02$ & $0.062\pm0.0$ & $0.82\pm0.04$ & $0.251\pm0.03$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{medium}  & False & $0.0\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.003\pm0.0$ & 5 \\ 
& True & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.022\pm0.0$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{open}  & False & $0.037\pm0.0$ & $0.01\pm0.0$ & $0.4\pm0.0$ & $0.143\pm0.01$ & 5 \\ 
& True & $0.029\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.107\pm0.01$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{umaze}  & False & $0.004\pm0.0$ & $0.001\pm0.0$ & $0.2\pm0.0$ & $0.059\pm0.0$ & 5 \\ 
& True & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.075\pm0.0$ & 5 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/maze/deterministic/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.66]{assets/query-eval/maze/deterministic/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{deterministic} in \emph{maze} environments } 
\label{fig:maze-deterministic}
\end{figure}

==> assets/query-eval/old-tables-with-std/maze/dynamics-type/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{dynamics-type} comparison in \emph{maze} environments } 
\label{table:maze-dynamics-type}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & dynamics-type & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{2}{3.6em}{large}  & autoregressive & $0.131\pm0.02$ & $0.06\pm0.0$ & $0.8\pm0.0$ & $0.233\pm0.05$ & 5 \\ 
& feed-forward & $0.14\pm0.02$ & $0.062\pm0.0$ & $0.82\pm0.04$ & $0.251\pm0.03$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{medium}  & autoregressive & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.031\pm0.0$ & 5 \\ 
& feed-forward & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.022\pm0.0$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{open}  & autoregressive & $0.034\pm0.0$ & $0.014\pm0.0$ & $0.5\pm0.0$ & $0.123\pm0.01$ & 5 \\ 
& feed-forward & $0.029\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.107\pm0.01$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{umaze}  & autoregressive & $0.007\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.07\pm0.0$ & 5 \\ 
& feed-forward & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.075\pm0.0$ & 5 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/maze/dynamics-type/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.66]{assets/query-eval/maze/dynamics-type/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{dynamics-type} in \emph{maze} environments } 
\label{fig:maze-dynamics-type}
\end{figure}

==> assets/query-eval/old-tables-with-std/maze/ensemble-count/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{ensemble-count} comparison in \emph{maze} environments } 
\label{table:maze-ensemble-count}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & ensemble-count & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{5}{3.6em}{large}  & 10 & $0.168\pm0.05$ & $0.051\pm0.01$ & $0.6\pm0.0$ & $0.307\pm0.07$ & 5 \\ 
& 20 & $0.149\pm0.04$ & $0.057\pm0.02$ & $0.78\pm0.07$ & $0.269\pm0.07$ & 5 \\ 
& 40 & $0.138\pm0.04$ & $0.056\pm0.01$ & $0.82\pm0.04$ & $0.264\pm0.05$ & 5 \\ 
& 80 & $0.146\pm0.02$ & $0.061\pm0.01$ & $0.82\pm0.04$ & $0.269\pm0.03$ & 5 \\ 
& 100 & $0.14\pm0.02$ & $0.062\pm0.0$ & $0.82\pm0.04$ & $0.251\pm0.03$ & 5 \\ 
\midrule 
\multirow{5}{3.6em}{medium}  & 10 & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.023\pm0.01$ & 5 \\ 
& 20 & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.024\pm0.01$ & 5 \\ 
& 40 & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.021\pm0.0$ & 5 \\ 
& 80 & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.022\pm0.0$ & 5 \\ 
& 100 & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.022\pm0.0$ & 5 \\ 
\midrule 
\multirow{5}{3.6em}{open}  & 10 & $0.033\pm0.0$ & $0.009\pm0.0$ & $0.48\pm0.04$ & $0.127\pm0.02$ & 5 \\ 
& 20 & $0.031\pm0.0$ & $0.01\pm0.0$ & $0.5\pm0.0$ & $0.117\pm0.02$ & 5 \\ 
& 40 & $0.03\pm0.0$ & $0.011\pm0.0$ & $0.5\pm0.0$ & $0.11\pm0.02$ & 5 \\ 
& 80 & $0.029\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.108\pm0.01$ & 5 \\ 
& 100 & $0.029\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.107\pm0.01$ & 5 \\ 
\midrule 
\multirow{5}{3.6em}{umaze}  & 10 & $0.011\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.073\pm0.01$ & 5 \\ 
& 20 & $0.009\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.074\pm0.0$ & 5 \\ 
& 40 & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.077\pm0.0$ & 5 \\ 
& 80 & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.075\pm0.0$ & 5 \\ 
& 100 & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.075\pm0.0$ & 5 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/maze/ensemble-count/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.6]{assets/query-eval/maze/ensemble-count/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{ensemble-count} in \emph{maze} environments } 
\label{fig:maze-ensemble-count}
\end{figure}

==> assets/query-eval/old-tables-with-std/maze/horizon/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{horizon} comparison in \emph{maze} environments } 
\label{table:maze-horizon}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & horizon & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{4}{3.6em}{large}  & 20.0 & $0.028\pm0.0$ & $0.021\pm0.0$ & $0.62\pm0.04$ & $0.059\pm0.0$ & 5 \\ 
& 30.0 & $0.118\pm0.01$ & $0.047\pm0.0$ & $0.8\pm0.0$ & $0.295\pm0.04$ & 5 \\ 
& 40.0 & $0.218\pm0.02$ & $0.087\pm0.0$ & $0.82\pm0.04$ & $0.321\pm0.03$ & 5 \\ 
& 50.0 & $0.16\pm0.02$ & $0.07\pm0.01$ & $0.92\pm0.04$ & $0.247\pm0.04$ & 5 \\ 
\midrule 
\multirow{4}{3.6em}{medium}  & 20.0 & $0.0\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.006\pm0.0$ & 5 \\ 
& 30.0 & $0.0\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.019\pm0.0$ & 5 \\ 
& 40.0 & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.032\pm0.0$ & 5 \\ 
& 50.0 & $0.001\pm0.0$ & $0.001\pm0.0$ & $0.2\pm0.0$ & $0.031\pm0.0$ & 5 \\ 
\midrule 
\multirow{4}{3.6em}{open}  & 20.0 & $0.005\pm0.0$ & $0.001\pm0.0$ & $0.2\pm0.0$ & $0.029\pm0.0$ & 5 \\ 
& 30.0 & $0.015\pm0.0$ & $0.007\pm0.0$ & $0.5\pm0.0$ & $0.104\pm0.01$ & 5 \\ 
& 40.0 & $0.036\pm0.0$ & $0.016\pm0.0$ & $0.6\pm0.0$ & $0.119\pm0.01$ & 5 \\ 
& 50.0 & $0.062\pm0.0$ & $0.025\pm0.0$ & $0.6\pm0.0$ & $0.148\pm0.01$ & 5 \\ 
\midrule 
\multirow{4}{3.6em}{umaze}  & 20.0 & $0.0\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.007\pm0.0$ & 5 \\ 
& 30.0 & $0.0\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.012\pm0.0$ & 5 \\ 
& 40.0 & $0.006\pm0.0$ & $0.002\pm0.0$ & $0.2\pm0.0$ & $0.048\pm0.0$ & 5 \\ 
& 50.0 & $0.035\pm0.0$ & $0.008\pm0.0$ & $0.4\pm0.0$ & $0.195\pm0.01$ & 5 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/maze/horizon/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.63]{assets/query-eval/maze/horizon/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{horizon} in \emph{maze} environments } 
\label{fig:maze-horizon}
\end{figure}

==> assets/query-eval/old-tables-with-std/maze/mixture/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{mixture} comparison in \emph{maze} environments } 
\label{table:maze-mixture}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & mixture & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
large & False & $0.14\pm0.02$ & $0.062\pm0.0$ & $0.82\pm0.04$ & $0.251\pm0.03$ & 5 \\ 
\midrule 
medium & False & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.022\pm0.0$ & 5 \\ 
\midrule 
open & False & $0.029\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.107\pm0.01$ & 5 \\ 
\midrule 
umaze & False & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.075\pm0.0$ & 5 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/maze/mixture/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.7]{assets/query-eval/maze/mixture/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{mixture} in \emph{maze} environments } 
\label{fig:maze-mixture}
\end{figure}

==> assets/query-eval/old-tables-with-std/maze/normalization/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{normalize} comparison in \emph{maze} environments } 
\label{table:maze-normalize}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & normalize & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{2}{3.6em}{large}  & False & $0.215\pm0.03$ & $0.067\pm0.01$ & $0.82\pm0.04$ & $0.402\pm0.04$ & 5 \\ 
& True & $0.14\pm0.02$ & $0.062\pm0.0$ & $0.82\pm0.04$ & $0.251\pm0.03$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{medium}  & False & $0.0\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.017\pm0.0$ & 5 \\ 
& True & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.022\pm0.0$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{open}  & False & $0.033\pm0.0$ & $0.014\pm0.0$ & $0.5\pm0.0$ & $0.108\pm0.0$ & 5 \\ 
& True & $0.029\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.107\pm0.01$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{umaze}  & False & $0.003\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.047\pm0.0$ & 5 \\ 
& True & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.075\pm0.0$ & 5 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/maze/normalization/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.66]{assets/query-eval/maze/normalization/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{normalize} in \emph{maze} environments } 
\label{fig:maze-normalize}
\end{figure}

==> assets/query-eval/old-tables-with-std/maze/prior-scale/eval_metrics.tex <==
\begin{table}[h!]
\caption{Evaluation metrics for  \emph{prior-scale} comparison in \emph{maze} environments } 
\label{table:maze-prior-scale}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & prior-scale & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{2}{3.6em}{large}  & 0 & $0.14\pm0.02$ & $0.062\pm0.0$ & $0.82\pm0.04$ & $0.251\pm0.03$ & 5 \\ 
& 5 & $0.104\pm0.02$ & $0.051\pm0.01$ & $0.82\pm0.04$ & $0.197\pm0.02$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{medium}  & 0 & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.022\pm0.0$ & 5 \\ 
& 5 & $0.0\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.02\pm0.0$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{open}  & 0 & $0.029\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.107\pm0.01$ & 5 \\ 
& 5 & $0.032\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.115\pm0.01$ & 5 \\ 
\midrule 
\multirow{2}{3.6em}{umaze}  & 0 & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.075\pm0.0$ & 5 \\ 
& 5 & $0.006\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.071\pm0.0$ & 5 \\ 
\bottomrule 
\end{tabular}
\end{sc}
\end{footnotesize} 
\end{center} 
\end{table}


==> assets/query-eval/old-tables-with-std/maze/prior-scale/sr_coverage.tex <==
\begin{figure}[!h]
\centering
\includegraphics[scale=0.66]{assets/query-eval/maze/prior-scale/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{prior-scale} in \emph{maze} environments } 
\label{fig:maze-prior-scale}
\end{figure}

==> assets/query-eval/old-tables-with-std/maze/uncertainty-type/eval_metrics.tex <==

\begin{table}[h!]
\caption{Evaluation metrics for  \emph{uncertainty-type} comparison in \emph{maze} environments } 
\label{table:maze-uncertainty-type}
\begin{center} 
\begin{footnotesize} 
\begin{sc} 
\scalebox{1}{
\begin{tabular}{|l | c | c | c| c | c | c |}
\toprule
Env. & uncertainty-type & AURCC$(\downarrow)$ & RPP$(\downarrow)$ & $CR_K(\uparrow)$ &  loss$(\downarrow)$ & runs \\
\midrule
\multirow{3}{3.6em}{large}  & ev & $0.14\pm0.02$ & $0.062\pm0.0$ & $0.82\pm0.04$ & $0.251\pm0.03$ & 5 \\ 
& pci & $0.139\pm0.02$ & $0.037\pm0.02$ & $0.42\pm0.1$ & $0.218\pm0.03$ & 5 \\ 
& u-pci & $0.155\pm0.02$ & $0.048\pm0.01$ & $0.46\pm0.05$ & $0.218\pm0.03$ & 5 \\ 
\midrule 
\multirow{3}{3.6em}{medium}  & ev & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.022\pm0.0$ & 5 \\ 
& pci & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.009\pm0.0$ & 5 \\ 
& u-pci & $0.001\pm0.0$ & $0.0\pm0.0$ & $0.2\pm0.0$ & $0.009\pm0.0$ & 5 \\ 
\midrule 
\multirow{3}{3.6em}{open}  & ev & $0.029\pm0.0$ & $0.012\pm0.0$ & $0.5\pm0.0$ & $0.107\pm0.01$ & 5 \\ 
& pci & $0.057\pm0.0$ & $0.012\pm0.0$ & $0.38\pm0.04$ & $0.168\pm0.01$ & 5 \\ 
& u-pci & $0.05\pm0.0$ & $0.012\pm0.0$ & $0.4\pm0.0$ & $0.168\pm0.01$ & 5 \\ 
\midrule 
\multirow{3}{3.6em}{umaze}  & ev & $0.008\pm0.0$ & $0.002\pm0.0$ & $0.3\pm0.0$ & $0.075\pm0.0$ & 5 \\ 
& pci & $0.035\pm0.0$ & $0.001\pm0.0$ & $0.2\pm0.0$ & $0.084\pm0.0$ & 5 \\ 
& u-pci & $0.017\pm0.0$ & $0.001\pm0.0$ & $0.2\pm0.0$ & $0.084\pm0.0$ & 5 \\ 
\bottomrule 
\end{tabular}
}
\end{sc}
\end{footnotesize} 
\end{center} 
\vspace{-10cm}
\end{table}


==> assets/query-eval/old-tables-with-std/maze/uncertainty-type/sr_coverage.tex <==
\begin{figure}[h!]
\centering
\includegraphics[scale=0.7]{assets/query-eval/maze/uncertainty-type/sr_coverage.png}
\caption{Selective-risk coverage curves for  \emph{uncertainty-type} in \emph{maze} environments } 
\label{fig:maze-uncertainty-type}
\end{figure}
